Resolving the jeans mass in hydrodynamic simulations of hierarchical clustering

We examine the necessity of resolving the Jeans mass in hydrodynamical simulations of the hierarchical formation of cosmological structures. We consider a standard two-component fluid and use smoothed particle hydrodynamics to model the baryonic component. It is found that resolution of the Jeans mass is not necessary to extract bulk properties of bound objects that are independent of resolution, provided that the objects have undergone a number of merger events. The degree of merging must be sufficient to populate the objects with substructure of similar total mass. After this criterion is met, neither the density profiles of structures nor their density-temperature distributions depend appreciably on the resolution of the simulation. Resolution of the Jeans mass by the imposition of a minimum temperature is not found to adversely affect the state of the matter in the final clusters. The baryon concentration profiles still indicate a deficit of gas with respect to the dark matter in the interiors of structures.

==> Figures/figure_captions.tex <==
\renewcommand{\thisdir}{Figures}

\figcaption[\thisdir/figs/Fig_1.eps]{
Temperature {\it vs.} gas density at a timescale factor, $a=0.17 a_f$.  The upper set of panels are for all the gas while the lower set is for a selected cluster.  From left to right, the panels correspond to simulations with increasing resolutions of $32^3$, $64^3$, and $128^3$ baryon particles.  The simulation data were resampled before analysis to the same mass resolution as the $32^3$ simulation. Contour lines in the upper panels are of constant mass surface density in $\rho-T$ space.  In the lower set of panels, the data points are for the sample of particles in the selected cluster.
\label{fig.Results.TvsRho_3Res}
}

\figcaption[\thisdir/figs/Fig_2.eps]{
The mean dark matter and gas density profiles.  The panel to
the left corresponds to the low resolution set of runs, while the
panel on the right is for the high resolution set.  Profiles are given
for clusters formed in the absence of a minimum temperature and for
clusters formed in a simulation with a minimum temperature scaled appropriately for the mean gas density at each epoch.
\label{fig.Results.RhoProfiles}
}

\figcaption[\thisdir/figs/Fig_3.eps]{
The distribution of gas density at early and late epochs. The upper set of panels is for the $32^3$ set of data while the lower set is for the $64^3$ set.  From left to right, the panels correspond to no minimum temperature and a minimum temperature scaled appropriately for the epoch.
\label{fig.Results.RhoDist}
}


\figcaption[\thisdir/figs/Fig_4.eps]{
Temperature {\it vs.} gas density for all the gas at an
expansion factor of $a=0.22 a_f$.  The circles in the right-hand panels
indicate the starting density and temperature.  For the left-hand
panels, these points are off the figure at $T=100\K$. The lines projecting
to the lower left of each circle correspond to the path of taken by a
uniform gas expanding and cooling adiabatically (lower line) and to
the path of gas maintaining $T_{min}$ (upper line).  The panels are arranged as in \fig{fig.Results.RhoDist}.
\label{fig.Results.TvsRho_0.1}
}

\figcaption[\thisdir/figs/Fig_5.eps]{
Temperature {\it vs.} gas density for all the gas at an expansion factor of $a=a_f$. The panels are as described in \fig{fig.Results.TvsRho_0.1}.
\label{fig.Results.TvsRho_1}
}

\figcaption[\thisdir/figs/Fig_6.eps]{
Temperature {\it vs.} gas density for the gas of a single cluster at an expansion factor, $a=a_f$. The panels are as described in \fig{fig.Results.TvsRho_0.1}.
\label{fig.Results.TvsRho_cluster_1}
}

\figcaption[\thisdir/figs/Fig_7.eps]{
The radial profile of the mean baryon fraction parameter, $\Upsilon$, for the clusters formed at different resolutions in the presence or absence of a minimum temperature.
\label{fig.Results.BFProfiles}
}


==> Figures/figures/fig.Results.TvsRho_cluster_0.1.tex <==
\begin{figure}
\plotone{\thisdir/figs/TvsRho.zoom_t=0.1.eps}
\caption{Temperature {\it vs.} gas density for the gas of a single cluster at an expansion factor, $a=0.22 a_f$.  The panels are arranged as in \fig{fig.Results.RhoDist}.}
\label{fig.Results.TvsRho_cluster_0.1}
\end{figure}

